CPopQA: Ranking Cultural Concept Popularity by LLMs

Prior work has demonstrated large language models' (LLMs) potential to discern statistical tendencies within their pre-training corpora. Despite that, many examinations of LLMs' knowledge capacity focus on knowledge explicitly appearing in the training data or implicitly inferable from similar contexts. How well an LLM captures the corpus-level statistical trends of concepts for reasoning, especially long-tail ones, is still underexplored. In this study, we introduce a novel few-shot question-answering task (CPopQA) that examines LLMs' statistical ranking abilities for long-tail cultural concepts (e.g., holidays), with a specific focus on these concepts' popularity in the United States and the United Kingdom, respectively. We curate a dataset containing 459 holidays across 58 countries, generating a total of 6,000 QA testing pairs. Experiments on four strong LLMs show that large models are capable of ranking long-tail cultural concepts regarding their statistical tendency. Notably, GPT-3.5 displayed superior performance and exhibited its potential to identify geo-cultural proximity across continents.

==> sections/02_related.tex <==
\section{Related Work}
\label{sec:related}

% Mansi to fill in
In recent years, Natural Language Processing (NLP) has evolved at a faster pace with applications such as virtual assistants, customer support chatbots, and the most recent one, ChatGPT from OpenAI. We have studied multiple papers where question answering (QA) in NLP has garnered significant attention. Researchers have studied and experimented with multiple model architectures, such as transformer-based models like BERT and GPT which have given promising results in QA tasks. Considering the different requirements and scenarios, several QA types have been used on a dataset. We focus our research work on QA systems, the different sets of datasets used for the QA and ranking-based question answering.

Free-form Table Question Answering dataset (FeTaQA) introduced a new dataset derived from Wikipedia, consisting of 10,000 pairs of {table, question, free-form answer, supporting table cells}, focusing on natural language QA (Linyong et al., 2022). In a study on language models for QA (Jiang et al., 2021) explored multiple-choice QA on science-based datasets like ARC, AI2, and Openbook QA, as well as extractive QA on SQuAD dataset based on Wikipedia articles. STRATEGYQA (Geva et al., 2021) was developed using a dataset generation procedure involving term-based priming and controlled annotator population, resulting in strategy questions, decompositions, and evidence paragraphs for multiple-choice QA tasks. QED (Lamm et al., 2021) focused on posthoc explanation generation based on given answer and the simultaneous generation of both question answers and explanations using Google Natural Question Dataset. Clark et al. (2020) presented TYDI QA, a multilingual question answering dataset based on Wiki articles. CoQA (Reddy et al., 2019), a conversational question answering that evaluated dialogue and reading comprehension models on a dataset containing 127k questions with answers from diverse domains such as Science, Literature, News, Wiki, and Reddit. Another study across such multiple domains included the dataset of having ~110,000 Quizbowl (Wallace et al., 2019) questions in natural language form, validated through models and live human evaluation. Choi et al. (2018) explored QuAC, a contextual question answering type, using a dialog-style dataset consisting of conversations between students and teachers to provide context for question answering tasks.

Culturally based datasets mainly included the study on multilingual question answering, with datasets created for diverse languages. These datasets enabled the development of models for extracting QAs, contextual QAs, mixed QAs, or visual QAs, depending on the specific domain of study (Becattini et al., 2023; Longpre et al., 2021).

The field of ranking-based question answering has received limited attention in the existing research literature. Transformer-based answer selection models have been explored for retrieval and ranking based approaches, but they are limited in considering question relevancy and may neglect suboptimal answers. Zhang et al. (2023) proposed a double retrieval and reranking model that overcomes these limitations and achieves better results on datasets such as WikiQA, TREC-QA, SelQA, and HotpotQA, which consist of natural questions with answer candidates. KBQA (Wang et al., 2021), knowledge-based question answering, where author experimented with similar framework using BERT model, achieving improved performance on datasets like SimpleQuestions and FreeBase QA. The few other studies have focused on fine-tuning models for ranking tasks and conducting analysis on evaluation metrics (Jans et al., 2012; Qiao et al., 2019). In contrast, our work aims to address ranking-based statistical QA on a culturally diverse dataset specifically focused on holidays from 58 countries.

%

==> tables/US_Freq_QAs.tex <==
\begin{table*}[!h]
\centering
\resizebox{0.98\columnwidth}{!}{%
\begin{tabular}{|p{5cm}|p{2.5cm}|p{4cm}|p{5cm}|}
\hline
\textbf{Question} & \textbf{Answer} & \textbf{Holiday Popularity} & \textbf{Description} \\
\hline
% Can you provide a descending order for the following Mexican holidays by their popularity in the United States: Columbus Day, Epiphany, Father's Day, Mother's Day, Christmas Day? & 1. Christmas Day
% 2. Epiphany
% 3. Mother's Day
% 4. Columbus Day
% 5. Father's Day & The percentage of the frequency of the holiday Columbus Day mentioned in the United States corpus is 1.21e-07... & Columbus Day: Columbus Day is a national holiday in many countries of the Americas and elsewhere, and a federal holiday in the United States... \\
% \hline
Can you provide a descending order for the following Chinese holidays by their popularity in the United States: Labour Day, Victory over Japan Day, Martyrs' Day, Army Day, Dragon Boat Festival? & 1. Army Day 
2. Labour Day 
3. Dragon Boat Festival 
4. Martyrs' Day 
5. Victory over Japan Day & The percentage of the frequency of the holiday Labour Day mentioned in the United States corpus is 1.17e-08... & Labour Day: International Workers' Day, also known as Labour Day in some countries and often referred to as May Day, is a celebration of labourers and the working classes... \\
\hline
Can you provide a descending order for the following Indian holidays by their popularity in the United States: Independence Day, Gandhi Jayanti, Bihu, Accession Day, Day of Ashura? & 1. Independence Day
2. Accession Day
3. Bihu
4. Day of Ashura
5. Gandhi Jayanti & The percentage of the frequency of the holiday Independence Day mentioned in the United States corpus is 4.07e-07... & Independence Day: Independence Day is celebrated annually on 15 August as a public holiday in India commemorating the nation's independence from the United Kingdom... \\
\hline
Can you provide a descending order for the following American holidays by their popularity in the United States: Christmas, Halloween, Hanukkah, Holi, Easter? & 1. Christmas
2. Easter
3. Halloween
4. Holi
5. Hanukkah & The percentage of the frequency of the holiday Christmas mentioned in the United States corpus is 1.72e-05... & Christmas: Christmas is an annual festival commemorating the birth of Jesus Christ, observed primarily on December 25 as a religious and cultural celebration among billions... \\
\hline
% Can you provide a descending order for the following Persian holidays by their popularity in the United States: Tasua, Islamic Republic Day, Mission of Muhammad, Nowruz, Eid ul-Adha? & 1. Nowruz
% 2. Mission of Muhammad
% 3. Eid ul-Adha
% 4. Islamic Republic Day
% 5. Tasua & The percentage of the frequency of the holiday Tasua mentioned in the United States corpus is 1.02e-10... & Tasua: In the days of Tesua and Ashura, Shia Muslims go to mosques and Takiehs or go to mourning ceremonies... \\
% \hline
Can you provide a descending order for the following Fijian holidays by their popularity in the United States: New Year's Day, Ram Naumi, Fiji Day, National Youth Day, Palm Sunday? & 1. New Year's Day
2. Palm Sunday
3. National Youth Day
4. Fiji Day
5. Ram Naumi & The percentage of the frequency of the holiday New Year's Day mentioned in the United States corpus is 5.78e-07... & New Year's Day: In the Gregorian calendar, New Year's Day is the first day of the year; 1 January... \\
\hline
\end{tabular}
}
\caption{QA pair examples for 5-holiday ranking in the US.}
\label{tab:us_exps}
\end{table*}
